Topic Modeling the Reading and Writing Behavior of Information Foragers

The general problem of "information foraging" in an environment about which agents have incomplete information has been explored in many fields, including cognitive psychology, neuroscience, economics, finance, ecology, and computer science. In all of these areas, the searcher aims to enhance future performance by surveying enough of existing knowledge to orient themselves in the information space. Individuals can be viewed as conducting a cognitive search in which they must balance exploration of ideas that are novel to them against exploitation of knowledge in domains in which they are already expert. In this dissertation, I present several case studies that demonstrate how reading and writing behaviors interact to construct personal knowledge bases. These studies use LDA topic modeling to represent the information environment of the texts each author read and wrote. Three studies revolve around Charles Darwin. Darwin left detailed records of every book he read for 23 years, from disembarking from the H.M.S. Beagle to just after publication of The Origin of Species. Additionally, he left copies of his drafts before publication. I characterize his reading behavior, then show how that reading behavior interacted with the drafts and subsequent revisions of The Origin of Species, and expand the dataset to include later readings and writings. Then, through a study of Thomas Jefferson's correspondence, I expand the study to non-book data. Finally, through an examination of neuroscience citation data, I move from individual behavior to collective behavior in constructing an information environment. Together, these studies reveal "the interplay between individual and collective phenomena where innovation takes place" (Tria et al. 2014).

==> 2-corpus-management.tex <==
\chapter{Methods: Corpus Management}
\label{chapter:corpus-management}

\section{Dataset Curation}


\subsection{Data Provenance}
Data provenance is the lineage of a digital object.  It captures factors that influenced an item or artifact's creation and transformation including the actors, agents (algorithms) and datasets that were part of the transformation of a digital object from one state to another. Data provenance is critical to the asserting the trustworthiness of a digital data product, especially when time and/or distance separate the digital object from its creator \cite{Plale2016,provbook}. 

% The PROV Data Model is shown in Figure \ref{fig:prov-model}, emphasizing the rela \emph{htrc:hasCriterion},tionship between \emph{prov:Entity}, \emph{prov:Activity}, and \emph{prov:Agent}.

Data provenance captured during use of modeling can aid a researcher in numerous ways. A researcher can interact with a dataset over a period of weeks to months. Over that time, their workset may be continuously refined as content is added or removed. Provenance tracks these changes. As data analysis is carried out, new data products will be created, some of which will be exported as non-consumptive exports while others will be discarded as not of use. It is the role of provenance to track and connect this activity taking place over the duration of extended engagement of a researcher with their data set.

Over time, these analytical actions accumulate and exports are created.  The publishable end product of research can then be conceived as the set $R = \{exports, Workset, Provenance\}$ where $export$ is one or more exports deemed to be non-consumptive, $Workset$ is the workset created and refined by the user, and $Provenance$ is the record of activity that links $NC-export$, intermediate results, and the $Workset$. 

%\begin{figure}
%\includegraphics[width=0.5\textwidth]{img/prov-model.png}
%\caption{The PROV Data Model starting points, showing primary entity types and relations. The PROV-O guidelines specify additional relations, including ``qualified'' relations that enable precise description of these starting points. For example, the ``wasDerivedFrom'' relation could be qualified by a ``Revision'', ``Quotation'', or ``PrimarySource.'' Each of those qualified derivations may link to other Agents or Entities in the graph. \cite{W3C-PROV-O}}
%\label{fig:prov-model}
%\end{figure}

\section{Model of Integration}\label{sec:integrate}
The framework of workflow, workset, and data provenance within a Capsule provide a coherent way for researcher interaction both with their defined workset, and with the HTDL collection over which their analysis will be carried out. 

A key component of the framework is a RESTful API through which a workset is imported into and exported from a Capsule.  The workset is converted to a JSON-LD representation \cite{W3C-JSON-LD}. This API adheres to the Linked Data Platform (LDP) practices for publishing linked data \cite{W3C-LDP}. LDP has been implemented in several digital libraries, including the OCLC's WorldCat \cite{OCLC-LOD-book}, Digital Public Library of America\footnote{\url{https://dp.la/info/developers/map/}}, and Library of Congress\footnote{\url{http://ld.loc.gov/}}.  Workflows are annotated with the PROV ontology \cite{W3C-PROV-O}, which defines a common vocabulary for describing data provenance.
The components of this framework and their interaction is summarized in Figure~\ref{fig:workflow}. %The W3C PROV ontology \cite{W3C-PROV-Primer} is integrated into the HTRC Wrkset Ontology \cite{Jett2016}.

Using the topic modeling workflow example from earlier, we created functionality to automatically create a provenance graph for the topic analysis using the PROV standard \cite{W3C-PROV-Primer}. This provenance capture allows for proper attribution to the workset curator, to the researcher, and possibly to a third party running analysis algorithms on behalf of a research project. 

Through use of the vocabulary of the PROV ontology \cite{W3C-PROV-O}, we describe a workset as a \emph{prov:Collection}, declaring that each \emph{htrc:Workset} is a \emph{prov:Collection}. Each workflow, like the topic modeling workflow above, corresponds to a \emph{prov:Plan}. The actual commands run by the analysis are a \emph{prov:Activity}, while the artifacts created by an analysis are a \emph{prov:Entity}.  Each organization or person that contributes to an analysis is a \emph{prov:Agent}.

Figure \ref{fig:prov-example} shows an example provenance graph for the modeling stages of the workflow, following the plan \emph{te:topicexplorer}. Three actions are carried out: \emph{r1act}, \emph{r2act}, and \emph{r3act}, each corresponding to the tokenization, stoplisting, and training phases of the model, all of which are executed by a \emph{user}. The underlying workset is abstracted as the \emph{corpus} node. Files created by the tokenization and stoplisting process are specified by the \emph{prov:wasGeneratedBy} and \emph{prov:wasDerivedFrom} relations.

The training step (\emph{r3act}) shows the highest level of sophistication in the graph and highlights the potential utility of provenance. The training produces three topic models, the abstract entity of which are labeled as \emph{model10}, \emph{model20}, and \emph{model40}. The actual instantiated models are then tied to the training step by the \emph{prov:wasGeneratedBy} relation, showing how this specific instance of a model was trained. Through the \emph{r3act} \emph{prov:Activity}, we can see that these models were trained specifically on the \emph{r2} revision of the workset, which has been tokenized by \emph{r1act} and stoplisted by \emph{r2act}. Going further through the provenance graph associated with \emph{corpus} would reveal the partner institutions and scanning practices that went into creating the workset that the user analyzed.

All of this enables a quick way to validate and replicate results, tracking the software versions used to create the analysis and the command line arguments that were used. The PROV graph additionally aids in connecting non-consumptive exports to analysis activities and worksets, thus providing the fundamental principles and components needed for publishing of research done using the Data Capsule system.

\begin{figure*}
\includegraphics[width=0.94\textwidth]{img/2-corpus-workflow.png}
\caption{Sample provenance graph of topic modeling workflow. Actions displayed top-to-bottom in blue squares; research products as yellow ovals; users as orange pentagons. Graph follows visual conventions of the PROV Primer.}
\label{fig:prov-example}
\end{figure*}

==> img/1-introduction-diff.tex <==
\chapter{Introduction}
\label{chapter:introduction}

Scientific discovery, and knowledge acquisition more broadly, can be understood as two separate processes: \emph{the context of discovery} details the conception of a theory, while \emph{the context of justification} details the validation of a theory \citep{Reichenbach1938}. Both of these processes can be empirically observed. However, accounts of discovery often involve internal and underspecified cognitive processes (e.g., the ``Eureka!'' moment). This led philosophers of science to neglect the \protect\TLSins{context of} discovery, and focus instead on justification, which was more amenable to rational analysis \citep{sep-scientific-discovery}. To avoid these ``black boxes'' in the context of discovery, \citet{Simon1973} outlines that discovery is not a problem of induction: a normative logic of discovery measures the efficiency of methods for finding patterns in observations. This changes the problem in a key way: rather than finding a set of rules \emph{guaranteed} to find a discovery, a logic of discovery defines a procedure for discovery that can be compared with other procedures, similar to evaluating computational complexity of an algorithm. Rather than examining concepts or proofs, as in the context of justification, we evaluate the efficiency of a particular scheme at postulating new concepts. This conception of a normative logic of discovery is inspired by \citet{Hanson1958}'s \protect\TLSdel{\emph{hypothetico-deductive reasoning}.} \protect\TLSins{\emph{Patterns of Discovery}.} This style of reasoning is also known as ``abductive'' or ``retroductive'' reasoning. In abductive reasoning, the perceptual process of observation leads to the discovery of patterns. If these patterns could plausibly be explained by a hypothesis or scientific law, \protect\TLSdel{the} \protect\TLSins{then} that law is proposed (the abduction). Finally, the law can be verified through the usual (inductive) logic of justification \citep{Magnani2009,Mabsout2015}.

Moreover, discovery is more than acquiring new conceptual connections. Scientific discovery is inherently a social process \citep{Knorr1999}. Reading is one method of gathering knowledge from the broader culture, while writing \protect\TLSdel{writing} is a way to contribute back to that culture. By examining how an author's writings relate to other works published at the same time, we can move from individual behavior to collective behavior in constructing an information environment. Together, these two behaviors reveal ``the interplay between individual and collective phenomena where innovation takes place'' \citep{Tria2014}.


In this dissertation, I operationalize scientific discovery through several case studies of reading and writing behaviors. These behaviors implicitly reflect knowledge acquisition and knowledge creation. To measure changes in knowledge structures, I use LDA topic modeling (Chapter~\ref{chapter:topic-modeling}) to represent the information environment of the texts each author read and wrote. The differences between these texts can then be quantified using information-theoretic measures of semantic similarity (Chapter~\ref{chapter:info-theory}). In contrast to earlier studies of how individuals navigate information environments, I study \protect\TLSins{them} at the time scale of decades and years, rather than immediate information retrieval needs at the scale of minutes and seconds. These methods implicitly define a logic of discovery through the relation of readings in the information space to writings, which are the products of knowledge creation or scientific discovery.


In particular, I examine five case studies. Three case studies revolve around Charles Darwin. Darwin left detailed records of every book he read for 23 years, from disembarking from the H.M.S. Beagle to just after publication of \protect\TLSdel{The} \emph{\protect\TLSins{The} Origin of \protect\TLSdel{Species.} \protect\TLSins{Species}}\protect\TLSins{.} Additionally, he left copies of his drafts before publication. I characterize his reading behavior (Chapter~\ref{chapter:readings}), then show how that reading behavior interacted with the drafts and subsequent revisions of \protect\TLSdel{The} \emph{\protect\TLSins{The} Origin of \protect\TLSdel{Species} \protect\TLSins{Species}}  (Chapter~\ref{chapter:writings}), and expand the dataset to include later readings and writings (Chapter~\ref{chapter:extensions}). Then, through a study of Thomas Jefferson’s correspondence, I expand the study to non-book data. Finally, through an examination of neuroscience citation data, I start an investigation at the level of collective phenomena, examining discipline-wide production as opposed to individual readings. 



\section{Bounded Rationality}
People are limited in how much information they can process by the problem structure and by cognitive, temporal, and physical constraints. In response to these constraints, \citet{Simon1956} proposed that decision-makers are ``satisficers,'' searching for a satisfactory solution rather than an optimal solution. These satisfactory solutions are known as heuristics. While many classes of heuristics have been investigated for systematic errors and biases \citep{Kahneman1982}, these heuristics often lead to better decisions than optimal procedures \citep{Gigerenzer1999}. This is often due to reduced processing cost increasing the output rate. These ``fast and frugal'' methods have less computational complexity.





Information processing is bound by physical constraints of energy, time, and thermodynamics.  \citet{merkle_energy_1989} estimates that the human brain is capable of $10^{12}$ to $10^{15}$ logical operations per second, based on \citet{von_neumann_computer_2012}'s estimates of neural density and firing rates. However, these computational estimates do little to improve our understanding of cognition on the level of problem-solving behaviors. In an early seminal work on cognitive load, \citet{miller_magic_1956} declared working memory capacity to be ``the magical number 7, plus or minus 2.'' Work on \emph{schema construction} explored what kind of thing was being held in memory through ``chunking'' \citep{chase_perception_1973}, discovering differences in chunk size with expertise. Experts still held 7 plus-or-minus 2 chunks, but each expert's chunk consisted of more chess moves than a novice's chunk. Experimental paradigms on the timescale of microseconds to minutes have found multiple perceptual bottlenecks in information processing \citep{marois_capacity_2005,tombu_unified_2011}. These include recognition, retention, and response bottlenecks. Attention management is a significant concern for human-machine interaction, reviewed in \citet{wickens_engineering_2015}.

In this dissertation, I am interested in cognitive timescales of years and decades. I introduce the notion of ``biographically-plausible datasets,'' data sets of a scale that could be reasonably encountered by a single individual in a lifetime. Biographically-plausible datasets are a complement to big data approaches in cognitive science, discovering what reasonable bounds are for having ``enough'' data bootstrapped from a naturally-occurring data source, such as a digital library or Twitter feed \citep{jones_big_2016}. For reading data, we estimate reasonable bounds as follows: a person reading two books a week for 70 years (from 8 to the United States life expectancy of 78) would have read 7,280 books. This estimate is validated by the size of Thomas Jefferson's Library. Thomas Jefferson had 6,487 books in his early library that was donated to the Library of Congress, and 939 in his retirement library that was curated over 12 years. While it is not likely that Jefferson read all of these books, and there may be overlap in collections, the total of 7,426 is very close to our estimate of 7,280 books in a lifetime of reading. Darwin's reading list consisted of 1,315 titles over 23 years of records, so approximately 1.1 book/week, which is below the estimated data size. The most extreme example we have found is British Prime Minister William Gladstone, who claimed to have read 22,000 books, which is an outlier in what is biographically-plausible. These estimates are an aid in bootstrapping big data into reasonable samples of individual behavior, and expand our understanding of bounded cognition to long-term tasks.

\section{Case Studies}
While the bulk of empirical studies in cognitive science are concerned with measuring population-level effects due to experimental manipulations, case studies play an important role in driving cognitive theorizing, experimentation, and modeling. For example, the case of the memory-impaired patient H.M. has driven many advances in cognitive neuroscience and computational models of memory (reviewed in \citet{SquireWixted2011}).  Other case studies, such as that of the frontal-lobe injury in Phineas Gage, provide important contrasts for later studies (reviewed in \citet{Macmillan2000}). 

Detailed longitudinal investigations of a single individual may reveal changing strategies that cannot be observed in laboratory experiments involving a single trial. Cognitive science could be enriched by using longitudinal studies such as ours to design laboratory studies with higher ecological validity. However, it is a challenging task to design laboratory studies of (for example) reading choices that take into account a subject’s extensive prior history of reading decisions.

The case studies of Darwin, Jefferson, and citation networks presented in this dissertation utilize what \citet{goldstone_discovering_2016} call ``naturally-occurring data sets.'' These are the incidental records that are gathered from everyday interactions, such as census records, dictionaries, encyclopedias, financial transactions, tweets, patents, and citations. With the advent of ``big data'' in the broader scientific community, cognitive science is also leveraging these records for behavioral studies \citep{jones_big_2016}. Case studies provide an opportunity to validate big data studies, seeing if individual behavior matches aggregate behavior, potentially highlighting behavioral outliers and opportunities for model revision. While this dissertation focuses on individuals, Chapter~\ref{chapter:future} details some preliminary work to expand our studies to entire scientific disciplines.


\section{Search and Information Foraging}
Search is ``the behavior of seeking resources or goals under conditions of uncertainty.'' This broad definition begins the 2012 volume \emph{Cognitive Search: Evolution, Alogrithms, and the Brain} \citep{Todd2012}. Covering much more than use of a search engine, cognitive search is a fundamental component of human and non-human animal behavior. In the strongest view, all human problem solving can be understood as defining, refining, and resolving a search problem \citep{Newell1972}. Even without such a strong claim, search governs memory retrieval, spatial foraging, problem solving, scientific discovery, creativity, and perception from individual to group to societal cognition \citep{Hills2015}.

Individual scientists and scholars can be viewed as conducting a cognitive search in which they must balance \emph{exploration} of ideas that are novel to them against \emph{exploitation} of knowledge in domains in which they are already expert \citep{Berger-Tal2014}. This exploration-exploitation trade-off is a strategy for managing cognitive load. Researchers have studied the exploration-exploitation trade-off in cognitive search at timescales of minutes up to years and decades. Laboratory experiments on visual attention are one example of this balancing act on short timescales \citep{chun1996just}, while studies of the recombination of patented technologies demonstrate long-term group behavior \citep{Youn2014}. Human subject results on the exploration-exploitation trade-off are reviewed in \citet{Cohen2007}. These studies find that there is no general-purpose optimal solution to this trade-off. Rather than finding a single optimal solution with a stationary strategy, \citet{Berger-Tal2014} proposed that the exploration-exploitation trade-off is a dynamic system, varying with time to optimize towards a particular goal. This framework lists four major phases of exploration-exploitation trade-off over the course of an entire lifetime: \begin{enumerate}
\item \emph{Knowledge acquisition}, in which all energy resources are devoted to exploration;
\item \emph{knowledge accumulation}, in which the initial search landscape is exploited;
\item \emph{knowledge maintenance}, in which an satisfactory level of knowledge is maintained --- in other words, a satisficing stage that balances exploration with exploitation;
\item \emph{knowledge exploitation}, in which no new exploration occurs. 
\end{enumerate}
\noindent 


\subsection{Information Foraging Theory}
\emph{Information foraging theory} \citep{Pirolli1999} expands cognitive search to include an information environment about which agents have incomplete information. IFT ``aims to explain and predict how people will best shape themselves for their information environments and how information environments can best be shaped for people'' \citep{Pirolli2009}. The general problem of information foraging has been explored in many fields, including cognitive psychology \citep{Todd2012,Hills2015}, neuroscience \citep{Cohen2007}, economics \citep{March1991,Azoulay-Schwartz2004}, finance \citep{Uotila2009}, ecology \citep{Stephens1986,Eliassen2007}, and computer science \citep{Sutton1998}. In all of these areas, the searcher aims to enhance future performance by surveying enough of existing knowledge to orient themselves in the information space.

IFT draws upon the framework, theories, and models of optimal foraging theory (OFT) in biology \citep{Stephens1986}. OFT aims to explain how animals search for food, taking into consideration an organism's metabolism and the environmental structure. There are two primary variables optimized in OFT: $time$ and $energy$. In information foraging, $energy$ is analogous to $attention$:
\begin{quote}
When information consumes is rather obvious: it consumes the attention of its recipients. Hence a wealth of information creates a poverty of attention, and a need to allocate that efficiently among the overabundance of information sources that might consume it. \citep{Simon1971b}
\end{quote}

IFT has been developed through the rational analysis of the information foraging problem space, operationalizing foraging behaviors through use of the scatter-gather experimental model. This led to the creation of several models, including ACT-IF \citep{Pirolli1999}, MESA \citep{Miller2004}, CoLiDeS \citep{Kitajima2005}, and SNIF-ACT \citep{Pirolli2003,Fu2007}. Most of these models have studied how humans search for information on the World Wide Web, with positive results from applying OFT to model human behavior \cite{Pirolli2009,Fu2012}. This dissertation pushes these models beyond laboratory studies, using naturally-occurring, biographically-plausible datasets to quantify changes in foraging behavior between exploitation and exploration regimes.

\protect\TLSins{Information foragers decide what information to allocate attention to through \emph{information scent}, which is a general-purpose concept that refers to various indicators of information quality }\citep{chi_using_2001}\protect\TLSins{. Examples of information scent include summaries, such as those presented in web search results, in scientific abstracts, or on the jacket of a book; structured data, such as computer folders or cataloging information; and social cues, such as recommendations \citep{Pirolli2009}. Most measures of information scent are presented as goal-oriented. In the historical studies presented in this dissertation, we defer studies of information scent to future work.}


\section{Operationalization}
Our primary interest is in the texts that a particular author read and wrote. We modeled these texts using using Latent Dirichlet Allocation (LDA; \citet{Blei2003,Blei2012}), a type of probabilistic topic model. LDA is a generative model that represents each document as a bag of words generated by a mixture of topics. Furthermore, topic models predict the behavior of human subjects in a variety of word association and disambiguation tasks \citep{Griffiths2007}. Topic modelling goes beyond simple word-counting methods, because it captures the ways in which the meaning of words can shift given the contexts in which they occur.

LDA topic models have been extensively used to analyze human-generated text across many domains.  Our approach contrasts with previous uses of topic modeling to analyze the large-scale structure of scientific disciplines \citep{Griffiths2004,Hall2008,Blei2007,Cohen2015} and the humanities \citep{Poetics41, JDH, Jockers2013}, which are each created through the collective effects of individual-level behavior. 
Previous models of historical records have focused on language use as an indication of larger shifts in style \citep{Hughes2012,Underwood2012}, learnability \citep{hills2015recent}, or content \citep{Michel2011,Goldstone2014,Klingenstein2014} of significant portions of publications in a field, including a study of the journal \emph{Cognition} \citep{Cohen2015}. Our application of topic modeling to the works read by a single person is a novel way to quantify an individual's information environment.

Rather than proposing that an individual's exploration-exploitation behaviors are in response to an overall goal, behavior changes relative to the information environment. People make decisions about which text to read next and we quantify the relative surprise of these decisions, independent of their goal, using information theoretic measures. Work on quantifying semantic relations stretches back to \protect\TLSdel{Osgood's} \citet{Osgood1967}\protect\TLSins{'s} semantic \protect\TLSdel{differential \citeyear{Osgood1967}.} \protect\TLSins{differential.} The development of the vector space model, which represents documents were as weighted term frequency vectors, introduced the use of cosine distance for semantic similarity \citep{Salton1975}. As LDA topic models are a generative model, each document-topic distribution can be viewed as a source generating words for the document. This signal (the words) can be analyzed by information theoretic measures.

The first measure is the \emph{Kullback-Liebler divergence} (KL divergence) \citep{Kullback1951}. KL divergence measures the inefficiency of using one distribution to encode signals coming from a different distribution. \protect\TLSdel{For an example, see Figure~\ref{fig:kl-example}.}
KL divergence is asymmetric, a fact we leverage through a notion of \emph{enclosure} that determines whether one text is more comprehensive than another. In situations where a symmetric measure is preferred, for example in mutli-document comparisons or situations where temporal order is not a factor, we use the symmetrized KL divergence, known as the \emph{Jensen-Shannon divergence} (JSD) \citep{lin1991divergence}. The square root of the JSD is a true metric, known as the Jensen-Shannon distance \citep{Endres2003}. The JS divergence does not satisfy the triangle inequality, while the square root does \citep{fuglede2004jensen}. By analogy, KL divergence and JSD can be thought of as different answers to the question: ``how far away is the ski lodge?'' Answering with JSD is akin to answering with the distance in miles. Answering with KL divergence is akin to answering with the travel time, which may be different depending on whether you are going up or down the mountain. This dissertation formalizes these measures in Chapter~\ref{chapter:info-theory}.

The dissertation uses KL divergence as the basis for many different analyses between texts. When examining Darwin's reading history, we use the past-to-text and text-to-text divergence to quantify the amount of ``surprise'' in each reading decision, based on either the cumulative or immediate information environment. In the case of writing comparisons, we introduce the notion of \emph{enclosure}, which uses the asymmetries of the KL divergence to determine whether one text summarizes or is more comprehensive than another.

Our approach also views the exploration-exploitation trade-off as a dynamic process, but does not claim there is any goal-directed behavior driving these behavioral changes. Rather, exploration and exploitation behaviors change in response to the information environment intrinsic to the texts, and changing with the addition of new publications.



\section{Null Models for Case Studies}
As we utilize case studies, careful consideration must be given to a null model for significance testing. In our studies of reading behavior, we permute the order of each set of readings to generate possible reading orders. The selection at each reading date is constrained by the titles published at that date, as a book could not be read before its publication. In contrast to a null that includes permutations that neglect publication date, this restricted null captures the dynamics of publication in which a new work can unexpectedly change the information space. The process also avoids directly including a temporal variable in the textual model. In addition, using a sampling process over the same data set allows us to use the same topic model for each null, which in turn allows us to avoid making further decisions about topic model comparison. This model of reading permutations is used in Chapters~\ref{chapter:readings}, \ref{chapter:writings}, and \ref{chapter:extensions}.

In the case of writing behavior, we utilize a method known as ``query sampling'' to generate multiple topic distributions for each writing, based on the topics previously learned from a set of readings. This population of possible distributions is then compared to the reading topic distributions and to the distributions of other writings. The replications allow us to calculate a confidence interval for each distance computation, which also helps us assess fitness of the topic distributions for these out-of-sample texts \citep{Trosset2008}.

Cluster analysis of the topic distributions for each text reveal that query sampling generates stable ``intepretations'' governed by their dominant topic. For example, \emph{The Origin of Species} can be understood in terms of case studies (dominant topic about ``pigeons''), geography (dominant topic about various locations), or theory (dominant topic on ``development'', ``experiment'', ``geological''). Rather than being an indicator of the model's instability, this variability of outputs supports the historical interpretation of our case studies. In the humanities, the interpretation of texts is a central (if not \emph{the}) scholarly endeavor. Our approach does not claim a single ``correct'' interpretation, but rather a set of interpretations in dialog with one another. Digital methods augment existing debates in the humanities by providing quantitative evidence for different ways of examining a text \citep{Rockwell2016,Allen2017}. We explore these multiple interpretations in Chapter~\ref{chapter:writings}.

It is important to emphasize again that we make no teleological claims about the foraging behavior. Our null models do not inject any assumptions that Darwin was reading in order to write \emph{The Origin}. When speaking of an optimal information forager, we mean the shortest path within the information environment, not the shortest path in relation to another text, as measured by semantic similarity measures.

Finally, these null models are not common in cultural analytics, and stand as a contribution to the current state of the art. When looking at randomized samples from large datasets, the correlations in each null sample are distorted. By using randomized samples from a biographically-plausible data set, we maintain some of the correlations in the texts, meaning that differences from random selection must also overcome the correlations in the selections of the data set itself. This is clearly seen in the case of Darwin's readings, where the books were selected to investigate particular phenomena, so have intrinsic correlations, yet the path Darwin chose is less surprising than random selections among those books.


\section{Limitations}
Given the theoretical constructs of a logic of discovery, bounded cognition, and information foraging theory, this dissertation defers investigation of several key concepts to future work. One limitation of our methods is that bounded cognition is not explicitly treated in these case studies. There is no investigation of how attention was managed, only the assumption that it was and that we observe the consequences of that attention management in biographically-plausible datasets. \protect\TLSins{In Chapter~\ref{chapter:extensions}, we speculate on which books Darwin could have read by examining the content of his retirement library. Future work could also examine Darwin's ``books to be read'' list contained in the same notebooks we analyzed in Chapter~\ref{chapter:readings}.}

While these case studies are adjacent to the study of innovation and knowledge creation, we do not touch on the creative process---how ideas are combined to form new ones. While we affirm that works like \emph{The Origin of Species} are novelties, and show how they relate to the readings, we don't explain the writing process. Despite examining questions of cultural production, we don't draw distinctions between novelties and innovations, understood through \citet{boden2004creative}'s notion of \emph{p-creativity} and \emph{h-creativity}. In \emph{p-creativity} or personal creativity, a concept is new to an individual. In \emph{h-creativity} or historical creativity, a concept is new to an entire society. We only briefly touch on issues of precedence in an analysis of Alfred Russell Wallace's co-discovery of natural selection (Chapter~\ref{chapter:writings}).

Another limit is that while these case studies describe and operationalize different portions of a logic of discovery, we do not define a generative model that could itself stand as a logic of discovery. Exploratory work through a case study of over 100,000 authors in neuroscience and their publication abstracts is found in Chapter~\ref{chapter:future}. Similar to astronomy before the development of optics, long-term information foraging is in an era of theory-making and discovering what relevant phenomena should be observed. This dissertation is a step in that direction.



